Towards Multiscale Graph-based Protein Learning with Geometric Secondary Structural Motifs

Graph neural networks (GNNs) have emerged as powerful tools for learning protein structures by capturing spatial relationships at the residue level. However, existing GNN-based methods often face challenges in learning multiscale representations and modeling long-range dependencies efficiently. In this work, we propose an efficient multiscale graph-based learning framework tailored to proteins. Our proposed framework contains two crucial components: (1) It constructs a hierarchical graph representation comprising a collection of fine-grained subgraphs, each corresponding to a secondary structure motif (e.g., $\alpha$-helices, $\beta$-strands, loops), and a single coarse-grained graph that connects these motifs based on their spatial arrangement and relative orientation. (2) It employs two GNNs for feature learning: the first operates within individual secondary motifs to capture local interactions, and the second models higher-level structural relationships across motifs. Our modular framework allows a flexible choice of GNN in each stage. Theoretically, we show that our hierarchical framework preserves the desired maximal expressiveness, ensuring no loss of critical structural information. Empirically, we demonstrate that integrating baseline GNNs into our multiscale framework remarkably improves prediction accuracy and reduces computational cost across various benchmarks.

==> exp.tex <==



% We integrate our SSHG framework with GVP-GNN~\citep{jing2020learning}, ProNet-Backbone~\citep{wang2022learning}, Mamba~\citep{gu2023mamba}; see Appendix~\ref{appendix:mamba} for details. We name the model that integrates SSHG by adding `+SSHG' to models' name. We compare these integrating models
% against several existing models, including GCN~\citep{kipf2016semi}, IEConv~\citep{hermosilla2020intrinsic}, DWNN~\citep{li2022directed}, GearNet~\citep{zhang2022protein}, HoloProt~\citep{somnath2021multi}, GVP-GNN~\citep{jing2020learning}, and ProNet-Backbone~\citep{wang2022learning}, on benchmark tasks of enzyme reaction classification (React)~\citep{hou2018deepsf} and protein-ligand binding affinity prediction (LBA)~\citep{wang2004pdbbind,liu2015pdb}. 
% We use various metrics depending on the tasks e.g., mean absolute error (MAE), root mean square error (RMSE), and %~\citep{willmott2005rmse}, 
% Pearson Correlation~\citep{uebersax1987use}.
%We use percentage accuracy for classification tasks. 
%For prediction-related tasks, 

%classification dataset in Protein fold datasets (Fold) and Reaction classification datasets (React), and for protein classification on Computational prediction of protein-ligand binding affinity (LBA) dataset.
%\YH{Moreover, to capture the sequential information of the tokens discussed in \textbf{Section 5}, we integrate our fragmentation graph with Mamba~\citep{gu2023mamba}, see Appendix~\ref{appendix:mamba} for details}.
%\BW{These findings highlight the importance of incorporating both secondary structure information and comprehensive geometric features 
%through the integration of 
%via integrating equivariant frames in message passing.}
%, especially when dealing with large protein graphs.




%Enzymes, proteins that catalyze biological reactions, are classified using Enzyme Commission numbers (EC), which group them based on the reactions they catalyze~\citep{omelchenko2010non}. In this task, we evaluate the performance of EFGNN on enzyme reaction classification to highlight the advantages of incorporating secondary structure information and preserving geometric relationships between these structures. We use the same dataset and experimental setup as in~\citep{wang2022learning,hou2018deepsf}. Additional details on the dataset and the training, validation, and test splits are provided in Appendix~\ref{appendix:experiments}. As shown in Table~\ref{tab:react}, EFGNN outperforms existing models while significantly reducing training time.
%\ts{Are all methods where the average training time is displayed in Table 2 using the same number of epochs? If yes, we should say so. If not, the average time per epoch would have little meaning. The same question applies to the results shown in Table 3.} 

% Specifically, the training time is reduced by 46\% compared to the next best-performing model, representing a significant improvement in efficiency.
%This protein-related task confirms the advantage of EFGNN in boosting computational efficiency and classification accuracy. In Table~\ref{tab:react}, the results for the baseline methods come from \BW{XXX}, and we do not report the computational time if it is not available in the baseline papers. Also, we report the results for the baseline approaches for all remaining tasks. 


%The result undoubtedly further validates the points we made earlier.

% \YH


% We further showcase the advantage of EFGNNs against existing methods for the benchmark LBA task. 
% %Accurate protein-ligand binding affinity (LBA) 
% Accurate LBA prediction is crucial for drug discovery, as it guides the selection of promising drug candidates and reduces the need for costly and time-consuming experiments.
% We apply EFGNNs to this task, using the PDBbind dataset sourced from \citep{wang2004pdbbind,liu2015pdb} and following the experimental protocols established by~\citep{jing2020learning}, including its default dataset split with a 30\% identity threshold to assess the generalization capability of our models for unseen proteins; see Appendix~\ref{appendix:experiments} for more details of the dataset. 
% To assess how geometric information and secondary structure enhance the learning capacity and generalization of GNNs for LBA prediction, we evaluated the performance using statistical metrics, including RMSE, Pearson correlation and Spearman correlation, on the test dataset.
% Table~\ref{tab:lba} compares the performance of our approach (EFGNN and EFGraphMamba) against several existing popular approaches (including the existing SOTA approach like ProNet-Backbone \citep{wang2022learning}) in terms of accuracy across three different metrics and computational time. Again, our proposed EFGNN approaches not only outperform the baselines in terms of accuracy but also achieve better computational efficiency. 

%\textcolor{blue}{While, as shown in Table~\ref{tab:lba}, the performance is slightly lower than state-of-the-art models, we observed a significant improvement in training time. Interestingly, we found that the average number of edges involved in the fragmentation schemes for this dataset is relatively sparse, which we will discuss in more detail later.} 


%\BW{[The authors show that the forward pass of their network is faster compared to baselines, while achieving higher accuracy for protein reaction classification. On ligand binding affinity, however, they do not achieve high accuracy, but justify this by saying that the training time was low. However, what is convincing in such a case is Pareto optimality — showing either that for a given accuracy, EFGNN is fastest, or for a given computational budget, EFGNN is most accurate. Table 3 does not currently show this; for all we know, a smaller version of ProNet-Backbone might be faster and more accurate than EFGNN. {\bf Plot the curve: budget vs. accuracy}]}

%\BW{[For reaction classification and binding affinity regression, which fragment or set of fragments plays the most important role, respectively? An interpretability study on this could be beneficial.]}


%\BW{[A previous paper ``Learning Hierarchical Protein Representations via Complete 3D Graph Networks", from which they may have copied some of their results, seems to have conducted much more extensive experiments. It should be noted that the paper does not provide any indication of uncertainty for predictions or time measurements, such as error bars, which is a major flaw.]}


%\BW{[The author did not specify the size of the dataset used. I believe fragment-based methods are more useful when large protein/molecules are modeled. Another study on the model performance versus varying system sizes is necessary. The experiments are limited to proteins. Also, it is unclear to me either the all-atom proteins or only the backbone is used.]}


%\BW{[How does the model performance vary with different fragmentation dictionaries? Are the fragment sizes roughly balanced? If not, will this impact the performance? Additionally, will a simple K-Means clustering or spectral clustering also work?]}


%\BW{[EFGNN appears to be on par with IEConv in terms of test accuracy for protein reaction classification, though there is no indication of uncertainty. There does not seem to be a time measurement available for IEConv, even though the authors claim that EFGNN is superior in computational efficiency. For ligand binding affinity, EFGNN seems to perform worse than other methods in terms of RMSE and Pearson correlation. While EFGNN appears to be more computationally efficient than other methods, the advantage is not overwhelming; it might be faster, but not by orders of magnitude. Therefore, the analyses do not demonstrate EFGNN's superiority in prediction tasks, and its efficiency advantage is questionable.]}

%, similiar as those in previous sections. 
%These results suggest that capturing global information is essential for improving the generalization of GNN models, and SCHull's connectivity property ensures that the models effectively learn global geometry.


\iffalse
\vspace{-0.2cm}
\subsection{Discussion on Efficiency}
\vspace{-0.2cm}
\begin{wraptable}{r}{0.34\columnwidth} %[!ht]
\vspace{-1.2cm}
\centering
 \scriptsize
\begin{tabular}{lcc}
\toprule
     & Reaction & LBA \\
\midrule
 ProNet-Backbone & 7604 & 8414 \\
 EFGNN & 1273 & 3987 \\
\bottomrule
\end{tabular}\vspace{-0.2cm}
\caption{\footnotesize Average number of edges used for message passing by different models on reaction classification and LBA dataset. ProNet-Backbone utilizes radius cut off with default radius $10$\r{A} to construct the edges.}
\label{tab:efficiency}\vspace{-0.5cm}
\end{wraptable}
One of the key benefits of our method is its ability to significantly reduce training time. By utilizing a hierarchical graph structure, EFGNNs operate on smaller subgraphs during the message-passing process, which helps minimize the computational burden, particularly for large-scale protein graphs.

To illustrate this, we compare the average number of edges in the graphs used by ProNet-Backbone~\citep{wang2022learning} and those generated by our fragmentation approach for proteins across two benchmark datasets.
ProNet-Backbone constructs edges using a default radius cutoff of $10$\r{A}, linking residues within this distance in the protein. In contrast, our fragmentation approach first forms edges within each fragment and then adds edges between fragments on fragmentation graphs. The total number of edges for each protein in our method is then the sum of these intra-fragment and inter-fragment edges.

 As shown in Table~\ref{tab:efficiency}, in the React dataset, the average number of edges for our method is approximately 17\% of that in ProNet-Backbone, while our accuracy surpasses that of ProNet-Backbone, as demonstrated in Table~\ref{tab:react}.
In the LBA dataset, we observe that the average number of edges for our method is around 7\% of that in ProNet-Backbone.
\fi


%\BW{[There is no convincing evidence showing that the method is superior in terms of efficiency, as there might be trade-offs between accuracy and efficiency. The authors either did not provide efficiency metrics for other relevant methods with comparable accuracy, or they did not compare other methods with cheaper hyperparameters to make them as inaccurate as EFGNN, and then check if EFGNN is still more efficient.]}


%Our results consistently show substantial gains in computational efficiency without sacrificing state-of-the-art accuracy. 


%\subsection{\BW{Another Protein Related Tasks}}


%\vspace{-0.3cm}
%\subsection{\BW{ANOTHER PROTEIN TASK}}

%\BW{[For example, how do fragment-based neural networks that use equivariant methods other than frames perform? How about intra- and inter- fragment processing that aren’t equivariant at all? Alternatively, how about ablating the choice of fragmentation with another fragmentation method, or even a random fragmentation? As is, it is not clear where the “secret sauce” of the authors’ method is.]}


%In this section, we conduct ablation studies on different models to investigate the effects of several key components. Specifically, we compare models that use or omit our proposed fragmentation strategy, include or exclude geometric features, operate on dense versus sparse graph structures, adopt different architectures with a comparable number of parameters, and incorporate or omit SS tokens. These comparisons help us assess the contribution of each component to the overall performance. 
%All experiments are conducted on the EC reaction classification task. Each model is trained for $300$ epochs with a batch size of $16$. We report the average time per epoch and the peak memory usage during training in Table~\ref{tab:efficiency_comparison} and Table~\ref{tab:architecture_comparison}. For all models, we use four message passing blocks with different feature selection strategies, edge constructions and w/ or w/o secondary message passing; see Appendix~\ref{appendix:experiments_architectures} for architectural details.


\vspace{-0.2cm}
\subsection{Ablation Studies}
\vspace{-0.2cm}

In this section, we conduct ablation studies to investigate the impact of key components in our SSHG framework. Specifically, we examine: (1) the performance and efficiency trade-offs between existing dense or sparse radial graphs versus our SSHG-based construction, (2) architectural variations in the two-stage GNN design within SSHG under comparable parameter budgets, (3) the effect of using or omitting the hierarchical strategy, (4) the contribution of geometric features $g_i^\top g_j$, and (5) the impact of incorporating secondary structure (SS) information. These comparisons allow us to isolate the contribution of each component to the overall model performance. Tables~\ref{tab:efficiency_comparison} and \ref{tab:architecture_comparison} summarize the results of the first two factors.
However, due to space limitations, we defer the analysis of the last three factors— hierarchical strategy, geometric features, and SS information—to the appendix; see Table~\ref{tab:feature_selection} for details.
All experiments are performed on the EC reaction classification task, with each model trained for $300$ epochs using a batch size of $16$. We report test accuracy alongside training efficiency metrics, including average time per epoch and peak memory usage.  

Table~\ref{tab:feature_selection} shows that simply appending SS tokens as a feature to the original GNNs does not necessarily improve performance. In contrast, combining SS information and geometric features through a dedicated hierarchical mechanism leads to consistent improvements.

Table~\ref{tab:efficiency_comparison} provides a detailed comparison of training efficiency and resource usage across different graph learning strategies. For baseline models like ProNet and GVP-GNN, we observe that increasing the radial cutoff leads to denser graphs, which improves accuracy but at a steep computational cost. For instance, raising the cutoff from $4$ to $10$ increases the average number of edges more than tenfold (from ~1K to ~11K), resulting in significantly higher memory usage and longer training times. While this denser connectivity benefits model expressiveness, the trade-off in efficiency makes it less practical for large-scale protein datasets.
In contrast, our SSHG-based counterparts achieve comparable or better accuracy with significantly fewer edges, lower memory, and runtime costs. This efficiency comes from the hierarchical design, which separates local and global interactions. For example, ProNet-SSHG reaches $87.2$ accuracy using only ~1.6K edges—far fewer than the ~11K edges required by high-cutoff baseline models—demonstrating that structured sparsity can outperform dense connectivity.

Table~\ref{tab:architecture_comparison} examines the robustness of the SSHG framework to architectural choices, particularly the distribution of parameters between the two GNN stages. All tested configurations—whether balanced or skewed toward either stage—yield strong results, indicating that the SSHG design is flexible and stable. Interestingly, allocating more capacity to the first-stage GNN (responsible for residue-level encoding) slightly improves accuracy. This suggests that richer local representations contribute more significantly to downstream prediction than increasing the capacity of the global inter-structural stage alone.

Together, these ablation studies highlight a central strength of our SSHG framework: it enables higher accuracy with better computational efficiency, even under constrained resource settings. This makes SSHG highly suitable for scaling to large biomolecular datasets and for integration into real-world, time-sensitive applications like drug discovery and protein design.
% \begin{table}[!ht]
% \centering
% \fontsize{5.5}{5.5}\selectfont
% \begin{tabular}{lcccc}
% \toprule
%  & w/ fragment & w/ geometry  & Test Acc & Ave.Time (s/epoch) \\
% \midrule
% ProNet & \ding{55} & \ding{55} & 86.4 & 210 \\
% -- & \ding{51} & \ding{55} & 87.2 & 140 \\
% -- & \ding{51} & \ding{51} & 87.5 & 142 \\
% \midrule
% GVPGNN\citep{jing2020learning} & \ding{55} & \ding{55}  & 68.5 & 334 \\
% -- & \ding{51} & \ding{55}  & 71.5 & 234 \\
% -- & \ding{51} & \ding{51}  & 73.6 & 236 \\
% \bottomrule
% \end{tabular}
% \caption{\footnotesize Different GNNs w/ or w/o Fragmentation or Geometric information for EC reaction classification}
% \label{tab:my_label}
% \end{table}

\begin{table}[!ht]
\centering
\fontsize{7}{7}\selectfont
\begin{tabular}{l|ccc|c}
\toprule
 &w/ SS & w/ fragment & w/ geometry  & Test Acc  \\
\midrule
ProNet & \ding{55}  & \ding{55} & \ding{55} & 86.4  \\
-- & \ding{51}  & \ding{55} & \ding{55} & 87.0 \\
-- & -- & \ding{51} & \ding{55} & 87.2  \\
-- & -- & \ding{51} & \ding{51} & 87.5 \\
\midrule
GVPGNN\citep{jing2020learning} & \ding{55} & \ding{55} & \ding{55}  & 68.5 \\
-- & \ding{51} & \ding{55} & \ding{55}  & 66.7 \\
-- & -- & \ding{51} & \ding{55}  & 71.5  \\
-- & -- & \ding{51} & \ding{51}  & 73.6 \\
\bottomrule
\end{tabular}
\caption{\footnotesize \textbf{Feature Selection}: Different GNNs w/ or w/o Fragmentation, Geometric information or Secondary structure Tokens.
\SW{I believe this one will be moved to Appendix by us.}
}
\label{tab:feature_selection}
\end{table}

\begin{table}[!ht]
\centering
\fontsize{7}{7}\selectfont
\begin{tabular}{l|ccccc|c}
\toprule
 & w/ fragment & cutoff & Ave. Num Edges & Ave.Time (s/epoch) & Mem(MiB) & Test Acc\\
\midrule
ProNet & \ding{55} & 4 & 1034.5 & 138 & 1290 & 78.1  \\
-- & \ding{55} & 10 & 11316.8  & 210 & 14548 &  86.4\\
-- & \ding{51} & -- & 1593.3  & 140 & 1818 & 87.2\\  
\midrule
GVPGNN & \ding{55} & 4  & 1034.5  & 216 & 1558 & 65.5\\
-- & \ding{55} & 10 & 11316.8  & 334 & 8930 & 68.5\\
-- & \ding{51} & -- & 1593.3 & 236 & 1416 & 73.6\\
\bottomrule
\end{tabular}
\caption{\footnotesize \textbf{Efficiency Comparison}: Different GNNs are evaluated on dense or sparse graphs constructed using various edge construction methods.}
\label{tab:efficiency_comparison}
\end{table}

% \begin{table}[!ht]
% \centering
% \fontsize{5.5}{5.5}\selectfont
% \begin{tabular}{lcccc}
% \toprule
%   & SS & Test Acc & Ave.Time (s/epoch) \\
% \midrule
% ProNet & \ding{55} & 86.4 & 210 \\
% -- & \ding{51} & XXX & XXX \\  
% \midrule
% GVPGNN & \ding{55} & 68.5 & 334 \\
% -- & \ding{51} & XXX & XXX \\
% \bottomrule
% \end{tabular}
% \caption{\footnotesize Different GNNs+Fragmentation w/ or w/o geometric features/SS information for EC reaction classification. 'geo' \JF{What is 'geo' in reference to?} is short for geometric features.}
% \label{tab:my_label}
% \end{table}




==> img/atactic.tex <==
% Draw the atactic polystyrene structure
\chemfig{\vdots -[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]\vdots
}

\chemfig{\vdots -[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-[::90]*6(=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]\vdots
}

==> img/isotactic.tex <==
% Draw the atactic polystyrene structure
\chemfig{\vdots -[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]\vdots
}


==> img/syndiotactic.tex <==
\chemfig{\vdots -[2]CH(-*6([,,,,blue]=-=-=-))
-[2]CH_2-[2]CH(-[::90]*6(=-=-=-))
-[2]CH_2-[2]CH(-*6([,,,,blue]=-=-=-))
-[2]\vdots
}
